Enabling Fast Deep Learning on Tiny Energy-Harvesting IoT Devices

Energy harvesting (EH) IoT devices that operate intermittently without batteries, coupled with advances in deep neural networks (DNNs), have opened up new opportunities for enabling sustainable smart applications. Nevertheless, implementing those computation and memory-intensive intelligent algorithms on EH devices is extremely difficult due to the challenges of limited resources and intermittent power supply that causes frequent failures. To address those challenges, this paper proposes a methodology that enables fast deep learning with low-energy accelerators for tiny energy harvesting devices. We first propose $RAD$, a resource-aware structured DNN training framework, which employs block circulant matrix and structured pruning to achieve high compression for leveraging the advantage of various vector operation accelerators. A DNN implementation method, $ACE$, is then proposed that employs low-energy accelerators to profit maximum performance with small energy consumption. Finally, we further design $FLEX$, the system support for intermittent computation in energy harvesting situations. Experimental results from three different DNN models demonstrate that $RAD$, $ACE$, and $FLEX$ can enable fast and correct inference on energy harvesting devices with up to 4.26X runtime reduction, up to 7.7X energy reduction with higher accuracy over the state-of-the-art.

==> Chapters/Relatedwork.tex <==
\section{Related work}\label{related}
\vspace{-6pt}
%\noindent \textbf{Energy Harvesting}
%Researchers have proposed various system checkpointing techniques~\cite{ransford2012mementos} to store intermediate results to non-volatile memory (NVM) upon power failures~\cite{Jayakumar:2015:QUR:2810396.2700249,kawai20088kb,ransford2012mementos,5746342}. In addition, several studies~\cite{1573690,5746342,1175898} reported a processor design with ferroelectric non-volatile registers that have the access efficiency close to that of SRAM with superior endurance. Such non-volatile processors are ideal for energy-harvesting devices with their ability to more efficiently store the intermediate running states. 

%\noindent \textbf{AI on Edge}
Several works have been proposed to implement CNN on IoT devices. SONIC is an intermittence-aware software system with specialized support for DNN inference~\cite{intelBeyondEdge}. NeuroZERO introduces a co-processor architecture consisting of the main microcontroller that executes scaled-down versions of a (DNN) inference task~\cite{neuroZero}. A software/hardware co-design technique that builds an energy-efficient low bit trainable system is proposed in~\cite{lowbit}. Efficient memory aware data flow designs for inference are proposed~\cite{memwarednn}.
%Zygrade proposes a task scheduling framework for batteryless systems that flexibly execute deep learning tasks~\cite{zygarde}. 
% \noindent \textbf{Block-Circulant Matrix} 
%The block-circulant matrix is used for weight representation.
% Eyriss presents a novel dataflow, called row-stationary on a spatial architecture~\cite{Eyriss}. Tangram proposes dataflow optimizations to address the shortcomings of existing parallel dataflow techniques for tiled Neural Network accelerators~\cite{Tangram}. Flexflow presents a flexible dataflow architecture that can leverage the complementary effects among feature map, neuron, and synapse parallelism to mitigate the mismatch~\cite{Flexflow}. Dataflow in FPGA accelerations proposed a specific dataflow of hardware CNN acceleration to minimize the memory access and data movement while maximizing the resource utilization to achieve high performance~\cite{FPGA}. 
%TF-Net pipeline efficiently deploys sub-byte CNNs on microcontrollers~\cite{tfNet}. %An analytical memory bandwidth model for loop-nest optimization targeting architectures with application-managed buffers is proposed in~\cite{dataReuse}. CDFEDT compares the error detection techniques in embedded systems for seven different techniques~\cite{comparison}. 
Intermittent-Aware Neural Architecture Search for task based inference and Hardware Accelerated Intermittent inference is proposed in \cite{InNAS} and \cite{HAI}, respectively. ePerceptive is on-device CPU based inference \cite{eperceptive}, based-on SONIC\cite{intelBeyondEdge}. 
Different from the above works, this is the first work that explores BCM-based DNN algorithms on resource-constrained energy harvesting IoT devices. 
% \textcolor{red}{(Caiwen: I do not recognize any of these works used block circulant matrix. Please double check)}
\vspace{-5pt}
